Embodied Carbon Accounting through Spatial-Temporal Embodied Carbon Models

Embodied carbon is the total carbon released from the processes associated with a product from cradle to gate. In many industry sectors, embodied carbon dominates the overall carbon footprint. Embodied carbon accounting, i.e., to estimate the embodied carbon of a product, has become an important research topic. Existing studies derive the embodied carbon through life cycle analysis (LCA) reports. Current LCA reports only provide the carbon emission of a product class, e.g., 28nm CPU, yet a product instance can be manufactured from diverse regions and in diverse time periods, e.g., a winter period of Ireland (Intel). It is known that the carbon emission depends on the electricity generation process which has spatial and temporal dynamics. Therefore, the embodied carbon of a specific product instance can largely differ from its product class. In this paper, we present new spatial-temporal embodied carbon models for embodied carbon accounting. We observe significant differences between current embodied carbon models and our spatial-temporal embodied carbon models, e.g., for 7nm CPU the difference can be 13.69%.

==> 2-Background.tex <==
\section{Background AND RELATED WORK }
\subsection{Embodied Carbon}
\textit{Embodied carbon} is defined as the total carbon released from processes associated with a product and within the boundaries of cradle-to-gate, which includes all activities from material extraction, manufacturing, transportation, and end-of-life \cite{hammond2011embodied}. Many corporations now publicly publish their yearly ESG reports containing carbon emissions based on the Greenhouse Gas (GHG) protocol \cite{napoletano2022environmental}, which is mandated in certain countries \cite{warren2023upcoming,bashir2023promise}. The GHG protocol categorizes carbon emissions into three Scopes. Scope 1 carbon emissions derive from directly burning fuels and other chemicals, e.g., by company vehicles, furnaces, etc.; Scope 2 emissions derive from purchasing energy, e.g., from the electric grid; and Scope 3 emissions derive from all other aspects of a company’s value chain, including carbon emissions from manufacturing the products. Scopes 1 and 2 roughly represent a company’s or a product's operational carbon, while Scope 3 roughly represents its embodied carbon \cite{bashir2023promise}. In the computing system, operational carbon is mostly Scope 2 and comes from using the grid to power IT equipment, while embodied carbon mostly comes from the manufacturing of computing hardware \cite{gupta2022act,bashir2023promise}. Previous studies have shown that embodied carbon dominates in the carbon foot of computing systems \cite{gupta2022act}. For example, the embodied carbon (manufacturing) of iPhone 11 accounts for 79\% of its overall carbon footprint \cite{iphone11}. Therefore, accurate embodied carbon accounting is essential and meaningful.


Semiconductor manufacturing is an energy-intensive industry. Carbon emissions caused by the consumption of electrical energy in the manufacturing process of the semiconductor product (e.g., CPU) account for a significant part of its embodied carbon\cite{bardon2020dtco,gupta2022act}. More accurate embodied carbon accounting data on products will be important in not only enabling each company in a supply chain to get greener products from upstream entities but also incentivizing upstream entities to reduce their carbon emissions in manufacturing  \cite{bashir2023promise}. Different types of organizations may be concerned about embodied carbon at different granularities. Companies that publish annual ESG reports \cite{bose2020evolution} may be concerned with embodied carbon on a yearly scale. Consumers may be more concerned about the embodied carbon of the individual product they want to buy, which is on a smaller spatial-temporal scale. It was found that 44\% of consumers preferred to buy products with specific carbon information, while 43\% were willing to spend more money to buy products with relatively low carbon \cite{pandey2011carbon}.







% \begin{table}[]
% \caption{Energy structure in five regions}
% \label{table: ci_5regions}
% \scalebox{0.7}{
% \begin{tabular}{cccc}
% \toprule
% Region &
%   \begin{tabular}[c]{@{}c@{}}Low carbon \\ energy sources\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Average carbon intensity \\ (g/kWh)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Dominant sources \\ in low carbon energy\end{tabular} \\ \toprule
% Ireland       & 39\% & 346 & Wind                     \\
% United States & 40\% & 367 & Wind, Hydro, Solar        \\
% South Korea   & 30\% & 436 & Solar                    \\
% China         & 34\% & 531 & Hydro, Wind, Solar, Nuclear \\
% Taiwan        & 18\% & 561 & Solar          \\\toprule          
% \end{tabular}}
% \end{table}



% \begin{table}[]
% \caption{XXX}
% \scalebox{0.7}{
% \begin{tabular}{ccc}
% \toprule
% \multirow{2}{*}{Spatial (Low carbon energy)} & \multicolumn{2}{c}{Temporal (Variable renewable energy)} \\ \cline{2-3} 
%                    & Season          & Day             \\ \toprule
% Ireland (39\%)     & Climate (wind)  & Weather (wind)  \\
% United States (40\%)                         & Climate (wind/hydro/solar)  & Weather (wind/hydro/solar) \\
% South Korea (30\%) & Climate (solar) & Weather (solar) \\
% China (34\%)                                 & Climate (Hydro/wind/solar)  & Weather (hydro/wind/solar) \\
% Taiwan (18\%)      & Climate (solar) & Weather (solar) \\\toprule
% \end{tabular}}
% \end{table}


% \begin{table}[]
% \caption{Meta data for our model.}
% \scalebox{0.8}{
% \begin{tabular}{|c|c|c|}
% \hline
% Mata Data & Description                                                                               & Range                    \\ \hline
% s         & \begin{tabular}[c]{@{}c@{}}Product manufacturing \\ location\end{tabular}                 & Regions, Counties        \\ \hline
% t &
%   \begin{tabular}[c]{@{}c@{}}Product manufacturing \\ time\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Short-term (hourly, daily)\\ {[}for individual consumer{]}\\ Long-term (monthly, yearly)\\ {[}for the companies that publish \\ annual or quarterly ESG reports{]}\end{tabular} \\ \hline
% CI(s,t)   & \begin{tabular}[c]{@{}c@{}}Electricity carbon intensity \\ in manufacturing.\end{tabular} & 0-760 g per kWh          \\ \hline
% ef        & Carbon emission factor                                                                    & 0-760 g per kWh          \\ \hline
% ES(s,t)   & \begin{tabular}[c]{@{}c@{}}Electricity generated \\ by each sources\end{tabular}          & \textgreater{}= 0 kWh    \\ \hline
% EPG       & Fab energy per GB                                                                         & \textgreater{}= 0 kWh/GB \\ \hline
% MPS       & Procure materials                                                                         & 500 g/kWh per cm2       \\ \hline
% EPS       & Fab energy                                                                                & 0.8-3.5 kWh per cm2      \\ \hline
% SIZE      & Dize size                                                                                 & \textgreater{}= 0 cm2    \\ \hline
% BD        & Bit density                                                                               & \textgreater{}= 0 GB/cm2 \\ \hline
% \end{tabular}}
% \end{table}

\subsection{Related Work}

The basic methods of accounting for embodied carbon is life cycle analysis (LCA) developed by environmental scientists used to quantify the environmental footprint of products across life cycles \cite{menoufi2011life}. There are two classes of LCA tools. The first one (EIO-LCA \cite{carnegie2008economic}) estimates carbon emissions based on the economic cost of electronics, which is translated to carbon by a coarse, industry-wide scale factor. The drawback is that it calculates carbon footprint using coarse-grained information. The other class of LCA tools is developed using database-based approaches \cite{ecochain}, which take a system’s bill of materials as input to estimate its overall carbon footprint. However, database-based LCA tools build carbon emission data on older process technologies (e.g., 45nm), and the granularity of the databases is coarse \cite{SpheraLCA,gupta2022act}. Recently, carbon-related studies in computing focus on embodied carbon accounting and carbon-aware optimization. 

(1) ACT \cite{gupta2022act} estimates the platforms’ embodied emissions by aggregating the footprint of each IC (i.e., bottom-up), including processors, memories, and storage. For example, the embodied carbon of processors is based on the die size and carbon emitted per unit size manufactured, which depends on semiconductor fab parameters including fab yield, the electricity consumed per unit size manufactured, emissions per unit size from chemicals burned during hardware manufacturing, and emissions from procuring raw materials for fab manufacturing. Finally, the electricity consumed is converted to carbon using the carbon intensity of electricity. However, the embodied carbon of memory and storage is directly from the product environmental LCA report of hardware vendors (e.g., Western Digital, SK Hynix, etc.).

(2) Tannu, S. \cite{tannu2022dirty}collects the 94 SSD LCA reports and 24 HDD LCA reports and calculates the average embodied carbon of all SSD and HDD. Most of the LCA reports in this work are from computer assembling vendors (e.g., HP, DELL, etc.), which contain less information than the reports from hardware vendors. This work is beneficial to compare and understand the embodied carbon of the two types of storage on the whole, while the granularity is not fine enough for the optimization of carbon-aware systems.

(3) Köhler, S. \cite{kohler2023carbon} proposes a carbon-aware optimization for memory systems. It uses an average value of all DRAMs as total embodied carbon modeling for memory directly from industrial LCA reports. It uses the simulated electricity from different sources (e.g., wind, coal, etc.) to analyze operational carbon but ignores the effect on embodied carbon. The ignoring may result in incorrect optimization. 

Overall, the existing embodied carbon models for computing systems do not consider spatial-temporal information. This paper fills in this gap.


\textbf{The Renewable Energy in electricity.} 

\textit{power generation.}

To solve Worldwide energy crises and carbon emissions, many studies focus on how to integrate renewable energy sources into power generation efficiently. For example, Shafiullah \cite{shafiullah2016hybrid} developed a hybrid renewable energy integration system, which comprised a techno-economic model, to facilitate RE integration in the Capricornia region of Central Queensland, Australia. 

\textit{Operation optimization.}

As the integration of renewable energy into power generation results in the carbon intensity of electricity varying over time, many studies in the computing community focus on carbon-aware operation optimization. For example, CarbonScaler \cite{hanafy2023carbonscaler} optimizes the carbon footprint of cloud platforms by exploiting the temporal flexibility inherent in many cloud workloads by executing them in time periods with the greenest electricity supply and suspending them at other times.


\textbf{The Spatial-temporal accounting of carbon emission in the grid.}

\textbf{Spatial variability}. The carbon intensity of electricity varies spatially across countries and regions. In general, regions with a higher dependence on fossil fuels have a higher average carbon intensity than those with a high percentage of low-carbon energy (renewable and nuclear) \cite{maji2022dacf}. \textbf{Temporal variability}. Even within a region, the proportion of each energy source contributing to electricity production varies over time, which leads to the carbon intensity of electricity varying over time \cite{maji2022carboncast}. The temporal variability pattern is affected by the type of variable variable renewable energy (e.g., solar, wind). For example, the predominant source of renewable energy in Ireland is wind, which is seasonally dependent \cite{foley2020critical,garrido2020impact}. Therefore, the carbon intensity in Ireland can be low in the months when wind resources are abundant. On a smaller time scale (e.g., day), wind power is also affected by weather. For example, Storm Malik in Ireland enabled renewable generation to reach 88.72 percent during a day, the vast majority of which came from wind \cite{Kevin}.








==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

